The Devil is in the Details: Simple Remedies for Image-to-LiDAR Representation Learning

LiDAR is a crucial sensor in autonomous driving, commonly used alongside cameras. By exploiting this camera-LiDAR setup and recent advances in image representation learning, prior studies have shown the promising potential of image-to-LiDAR distillation. These prior arts focus on the designs of their own losses to effectively distill the pre-trained 2D image representations into a 3D model. However, the other parts of the designs have been surprisingly unexplored. We find that fundamental design elements, e.g., the LiDAR coordinate system, quantization according to the existing input interface, and data utilization, are more critical than developing loss functions, which have been overlooked in prior works. In this work, we show that simple fixes to these designs notably outperform existing methods by 16% in 3D semantic segmentation on the nuScenes dataset and 13% in 3D object detection on the KITTI dataset in downstream task performance. We focus on overlooked design choices along the spatial and temporal axes. Spatially, prior work has used cylindrical coordinate and voxel sizes without considering their side effects yielded with a commonly deployed sparse convolution layer input interface, leading to spatial quantization errors in 3D models. Temporally, existing work has avoided cumbersome data curation by discarding unsynced data, limiting the use to only the small portion of data that is temporally synced across sensors. We analyze these effects and propose simple solutions for each overlooked aspect.

==> _header.tex <==
% ---------------------------------------------------------------
% Include basic ECCV package
 
% TODO REVIEW: Insert your submission number below by replacing '*****'
% TODO FINAL: Comment out the following line for the camera-ready version
\usepackage[review,year=2024,ID=1155]{accv}
% TODO FINAL: Un-comment the following line for the camera-ready version
%\usepackage{eccv}

% OPTIONAL: Un-comment the following line for a version which is easier to read
% on small portrait-orientation screens (e.g., mobile phones, or beside other windows)
%\usepackage[mobile]{eccv}


% ---------------------------------------------------------------
% Other packages

% Commonly used abbreviations (\eg, \ie, \etc, \cf, \etal, etc.)
\usepackage{accvabbrv}

% Include other packages here, before hyperref.
\usepackage{graphicx}
\usepackage{booktabs}

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.

\usepackage{xcolor}

\input{def}
% ---------------------------------------------------------------
% Hyperref package

% It is strongly recommended to use hyperref, especially for the review version.
% Please disable hyperref *only* if you encounter grave issues.
% hyperref with option pagebackref eases the reviewers' job, but should be disabled for the final version.
%
% If you comment hyperref and then uncomment it, you should delete
% main.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).

% TODO FINAL: Comment out the following line for the camera-ready version
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=accvblue]{hyperref}
% TODO FINAL: Un-comment the following line for the camera-ready version
%\usepackage{hyperref}

% Support for ORCID icon
\usepackage{orcidlink}


==> figures/frame_gap.tex <==
\begin{figure}[!t]
\centering
    \caption{
    \textbf{Linear Probing results of different frame gaps.
    } 
\includegraphics[width=1\linewidth]{frame_gap.pdf}\vspace{-3mm}
\vspace{-0.3cm}
    }\label{figure:frame_gap}
\end{figure}

==> tables/robustness.tex <==
% \begin{table}[!t]
%     \caption{\textbf{Model's robustness under OoD scenarios.}}
%     \vspace{-3mm}
%     \centering
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{ccccccc}
%         \toprule
%          \multirow{2}{*}{Method} & \multicolumn{2}{c}{mCE$\downarrow$} &  \multicolumn{2}{c}{mRR$\uparrow$} &  \multicolumn{2}{c}{avg. mIoU$\uparrow$} \\
%          \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
%          & LP & Full  & LP & Full & LP & Full \\
%          \midrule
%         SLidR & 179.38 & 106.08 & 77.18  & 75.99 & 29.9 & 56.8 \\
%         Ours & \textbf{162.29} & 104.54 & \textbf{82.39} & 76.72 & \textbf{37.2} & 58.1 \\
%         Seal & 166.18 & \textbf{92.63} & 75.38 & \textbf{83.08} & 33.9 & \textbf{62.8} \\   
%         \bottomrule
%     \end{tabular}}
%     \vspace{-3mm}
%     \label{table:robustness}
% \end{table}
